Inducing And Probing Charge Migration In Molecular Systems

Technological advancements in generation of ultrafast and intense laser pulses have enabled the real-time observation and control of charge migration in molecules on their natural timescale, which ranges from few femtoseconds to several hundreds of attoseconds. Present thesis discusses the effect of symmetry on the adiabatic attosecond charge migration in different molecular systems. The spatial representation of the charge migration is documented by time-dependent electronic charge and flux densities. Furthermore, the induced charge migration is imaged via time resolved x-ray diffraction (TRXD) with atomic-scale spatiotemporal resolution in few cases.

==> HeadTail/certi.tex <==
\newpage
\thispagestyle{empty}
 \vspace*{2cm}
\begin{center}
\textbf{\Large\underline {Approval Sheet}}
\end{center}
\vspace{1cm}
This thesis entitled \textbf{Inducing and Probing Charge Migration in Molecular Systems} by \textbf{Sucharita Giri} (Roll No. 174123002) is approved for the degree of Doctor of Philosophy in Physics.

\begin{flushright}
\textbf{Examiners}\\
\-------------------------\\
\-------------------------\\
\-------------------------\\



\textbf{Supervisor}\\
Dr. Gopal Dixit

\textbf{Chairman}\\
\-------------------------\\


\end{flushright}

\begin{flushleft}
Date :\\
Place :
\end{flushleft}



==> HeadTail/certi_appro.tex <==
\newpage
\thispagestyle{empty}
\vspace*{2cm}
\begin{center}
	\textbf{\Large\underline {Thesis Approval}}
\end{center}
\vspace{1cm}
This thesis entitled \textbf{Inducing and Probing Charge Migration in Molecular Systems} by \textbf{Sucharita Giri} (Roll No. 174123002) is approved for the degree of Doctor of Philosophy in Physics.
\vskip2cm
\begin{flushright}
	\textbf{Examiners}\\
	\vspace{0.5in}
	Prof. Vandana Sharma\\
	\vspace{0.5in}
	Prof. Sumiran Pujari\\
	\vskip1cm
	\textbf{Supervisor}\\
	\vspace{0.5in}
	Prof. Gopal Dixit
	\vskip1cm
	\textbf{Chairman}\\
	\vspace{0.5in}
	Prof. Anindya Dutta\\
	
	
\end{flushright}

\begin{flushleft}
	Date : 10/04/2023\\
	Place : Mumbai
\end{flushleft}


